Definability of linear equation systems over groups and rings

Motivated by the quest for a logic for PTIME and recent insights that the descriptive complexity of problems from linear algebra is a crucial aspect of this problem, we study the solvability of linear equation systems over finite groups and rings from the viewpoint of logical (inter-)definability. All problems that we consider are decidable in polynomial time, but not expressible in fixed-point logic with counting. They also provide natural candidates for a separation of polynomial time from rank logics, which extend fixed-point logics by operators for determining the rank of definable matrices and which are sufficient for solvability problems over fields. Based on the structure theory of finite rings, we establish logical reductions among various solvability problems. Our results indicate that all solvability problems for linear equation systems that separate fixed-point logic with counting from PTIME can be reduced to solvability over commutative rings. Moreover, we prove closure properties for classes of queries that reduce to solvability over rings, which provides normal forms for logics extended with solvability operators. We conclude by studying the extent to which fixed-point logic with counting can express problems in linear algebra over finite commutative rings, generalising known results on the logical definability of linear-algebraic problems over finite fields.

==> appendices/finite-rings-structure-proofs.tex <==
Finite local rings can intuitively be thought of as the basic building blocks of finite commutative rings and we summarise some of their useful properties in the following proposition.

\setcounter{theorem}{5}

% --- Properties of local rings -----------------------------------------------
\propositionLocalRingsProperties*

\begin{proof} The first claim follows directly by the uniqueness of
the maximal ideal $m$. For the second part, assume $R$ is local but
contains a non-trivial idempotent $x$, i.e.\ $x (1-x) = 0$. But then
$x$ and $(1-x)$ are two non-units distinct from $0$, hence contained
in the maximal ideal of $R$ but $x + (1-x) = 1$, a contradiction. On
the other hand, if $R$ only contains trivial idempotents, then
every non-unit in $R$ is nilpotent, for assume that $x\not=0$ is a
non-unit which is not nilpotent, then $x^{n+km}=x^n$ for some $m,
n\geq 1$ and all $k \geq 1$. In particular,
\[ x^{nm} \cdot x^{nm} = x^n \cdot x^{nm-n} \cdot x^{nm} = x^{n+nm}
\cdot x^{nm-n} = x^n \cdot x^{nm-n} = x^{nm}.\]
Since $x^{nm}\not=1$ we have $x^{nm}=0$ which is a contradiction to
our assumption that $x$ is not nilpotent. With this, it is easy to
verify that also sums of non-units are nilpotent, which implies that
the set of non-units forms a unique maximal ideal in $R$.

For the third part, assume $x \in R$ is  idempotent. Then $(1-x)^2 =
(1 - 2x + x^2) = (1-x)$ so $(1-x)$ is also idempotent. Furthermore,
as $x(1-x) = 0$ we see that $x$ and $(1-x)$
are orthogonal, and since $x + (1-x) = 1$, any element $r \in R$
can be expressed as $r = rx + r(1-x)$, so we conclude that $R = x R
\oplus (1-x) R$.

%In particular we have that $R = x R \oplus (1-x) R$, since assume
%that for some $r,s \in R$ we have $x r = (1-x) s$, then $x^2 r = 0$
%and hence $x r = 0 = (1-x) s$.

Finally, let $R$ be local and suppose $\card{R} = p^k n $ where $p
\nmid n$. We want to show that $n =1$. Otherwise $I_p = \lbrace r \in
R \sep p^k r = 0 \rbrace$ and $I_n = \lbrace r \in R \sep n r = 0
\rbrace$ would be two proper distinct ideals.
Furthermore we show that $R = I_p \oplus I_c$: therefore let  $x,y \in
\Z$ with $x p^k + y n = 1$. Assume $p^k r = 0 = n r$, then $x p^k r +
y n r = 0$ and hence $r = 0$. On the other hand for each $r \in R$ we
have that $n r \in I_p, p^k r \in I_n$ and so $y n r + x p^k r = r \in
(I_p + I_n)$. We derive a contradiction to $R$ being local. 
\end{proof}

\setcounter{theorem}{7}

%--- Definability of the base -------------------------------------------------
\lemmaRingIdempotentBase*

\begin{proof}
We claim that $\ringBase{R}$ consists precisely of those non-trivial
idempotent elements of $R$ which cannot be expressed as the sum of two
orthogonal non-trivial idempotent elements. To establish this claim,
consider an element $e \in \ringBase{R}$ and suppose that $e = x + y$
where $x$ and $y$ are orthogonal non-trivial idempotents. It follows
that $e$ is different from both $x$ and $y$, since if $e = x$, say,
then $y = e - x = 0$ and similarly when $e = y$. Now $ex = xe = x(x+y)
= x^2 + xy = x$ and, similarly, $ey = y$. Since both $ex$ and $ey$ are
idempotent elements in $eR$, it follows that $ex, ey \in \lbrace 0, e
\rbrace$, since $eR$ is local with identity $e$ and contains no
non-trivial idempotents. But by the above we know that $ex = x \neq e$
and $ey = y \neq e$, so $ex = ey = x = y = 0$. This contradicts the
fact that $e = x + y$ is non-trivial, so the original assumption must
be false.

Conversely, suppose $x \in R$ is a non-trivial idempotent element that
cannot be written as the sum of two orthogonal non-trivial
idempotents. Writing $\ringBase{R} = \lbrace e_1, \dots, e_m \rbrace$,
we get that  
\[
	x = x (1) = x (e_1 + \cdots + e_m) = xe_1 + \cdots + xe_m.
\]

\noindent
Each $xe_i$ is an idempotent element of $e_iR$ and since $e_iR$ is
local, $xe_i$ must be trivial. Hence, there are distinct $f_1, \dots,
f_n \in \ringBase{R}$, with $n \leq m$, such that $x = f_1 + \cdots +
f_n$. But since $x$ cannot be written as a sum of two (or more)
non-trivial idempotents, it follows that $n = 1$ and $x \in
\ringBase{R}$, as claimed.

\makebreak

\noindent
Now it is straightforward to write down a first-order formula that
identifies exactly all non-trivial idempotent elements that are not
expressible as the sum of two non-trivial orthogonal idempotents. If
$R$ is local then trivially $\ringBase{R} = \{1\}$. To test for
locality, it suffices
by Proposition~\ref{proposition_local-rings-properties} to check
whether all idempotent elements in $R$ are trivial and this can be
expressed easily in first-order logic. 
\end{proof}

==> appendices/further-background.tex <==
We provide further background reading for the topics considered in this paper.

% -----------------------------------------------------------------------------
% Lindstrom quantifiers and extensions
% -----------------------------------------------------------------------------
\subsection{Lindstr\"om quantifiers and extensions}

Generalised quantifiers in the sense of Lindstr\"om~\cite{lindstroem66genQuantifiers} have been studied as a way to increase the expressiveness of a logic by a prescribed query. Let $\sigma = (R_1, \dots, R_l)$ be a vocabulary where each relation $R_i$ has arity $n_i$. Consider a class $\structClass K$ of $\sigma$-structures that is closed under isomorphism; that is, for $\sigma$-structures $\struct A$ and $\struct B$, if $\struct A \in \structClass K$ and $\struct A \isom \struct B$, then $\struct B \in \structClass K$. With $\structClass K$ we associate a \emph{Lindstr\"om quantifier} $\lindstrom K$ whose \emph{type} is the tuple $(n_1, \ldots, n_l)$. The \emph{arity} of the quantifier $\lindstrom K$ is the value of $\max\{ n_1, \dots, n_l\}$. For a logic $\logic L$, define the extension $\logic{L}(\lindstrom K)$ by closing the set of formulae of $\logic L$ by introducing the following formula-formation rule:

\begin{quote}
if $\phi_1, \dots, \phi_l$ are formulae of $\logic{L}(\lindstrom K)$, $\tup x_1, \dots, \tup x_l$ tuples of variables where $\tup x_i$ has length $n_i$, then the expression $\lindstrom{K} \tup x_1 \dots \tup x_l \qsep (\phi_1, \dots, \phi_l)$ is a formula of $\logic{L}(\lindstrom K)$ with all occurrences of $\tup x_i$ in $\phi_i$ bound.
\end{quote}

\noindent The semantics of the Lindstr\"om quantifier $\lindstrom K$ is defined such that
\begin{quote}
	$\struct A \models \lindstrom{K} \tup x_1 \dots \tup x_l \qsep (\phi_1, \dots, \phi_l)$ if and only if $(\univ A; \phi_1(\tup x_1)^\struct{A}, \dots, \phi_l(\tup x_l)^\struct{A}) \in \structClass K$,
\end{quote}

\noindent where $(\univ A; \phi_1(\tup x_1)^\struct{A}, \dots, \phi_l(\tup x_l)^\struct{A})$ is interpreted as a $\sigma$-structure. 

Similarly we can consider the extension of a logic $\logic L$ by a collection $\mathbf Q$ of Lindstr\"om quantifiers. The logic $\logic L(\mathbf Q)$ is defined by adding a rule for constructing formulae with the quantifier $Q$, for each $Q \in \mathbf Q$, to the list of formula-formation rules for $\logic L$. The semantics is defined by considering the semantics for each quantifier $Q \in \mathbf Q$, as above.

Often we consider families of quantifiers generated under some uniformity condition. Here we focus on the following notion of uniformity, due to Dawar~\cite{dawar95generalized}. Let $\structClass K$ be a class of structures over vocabulary $\sigma = (R_1, \dots, R_l)$. For each $m \in \N$, let $\sigma_m$ be the vocabulary $(R_{m,1}, \dots, R_{m,l})$ where the arity of $R_{m,i}$ is $m \cdot n_i$. Let $\structClass K_m$ be the class of $\sigma_m$-structures defined by
\[
	\structClass K_m \defeq \{ (A, S_1, \dots, S_l) \sep (A^m, S_1, \dots, S_l) \in \structClass K \},
\]

\noindent 
where $(A^m; S_1, \dots, S_l)$ is seen as a $\sigma$-structure with universe $A^m$. If $Q_m$ is the Lindstr\"om quantifier associated with $\structClass K_m$ then we say that the sequence $\uniformLindstrom K \defeq \{ Q_m \sep m \in \N \}$ is \emph{uniformly generated by $\structClass K$}. 

\begin{definition}[Uniform sequences of quantifiers]
A countable collection $\mathbf Q$ of Lindstr\"om quantifiers is a \emph{uniform sequence} if there is a class of structures $\structClass K$ such that $\mathbf Q = \uniformLindstrom K$.
\defnend
\end{definition}


% -----------------------------------------------------------------------------
%
% Linear Algebra
%
% -----------------------------------------------------------------------------
\subsection{Linear algebra}
\label{sec_linear-algebra}

A matrix is usually regarded as a rectangular grid of elements, with rows and columns given in a particular order. However, most natural matrix properties are well-defined if we consider a more generic notion of a matrix, where the rows and columns are indexed by arbitrary unordered sets. In this section we introduce \emph{unordered matrices} of this kind and review some basic linear algebra. 

% 
% Elementary linear algebra
% 
\subsubsection{Matrices and linear maps}

Let $R$ be a commutative ring. An \emph{$m \times n$ matrix over $R$} is a rectangular array of scalars from $R$, consisting of $m$ rows and $n$ columns. We write $m \times n$ for the \emph{dimension} of $A$. An $m \times n$ matrix is said to be \emph{square} (of order $n$) if $m = n$. We write $A = (a_{ij})_{1 \leq i \leq m, 1 \leq j \leq n}$ (or $A = (a_{ij})$ for short when the dimension of $A$ is clear from the context) to denote the matrix
\[
	A = 
	\begin{pmatrix}
		a_{11} 	& 	\cdots 	& 	a_{1n} 	\\
		\vdots	&	\ddots	&	\vdots	\\
		a_{m1} 	& 	\cdots 	& 	a_{mn} 	\\
	\end{pmatrix}.
\]

\noindent
When $R = F$ is a field, a matrix over $F$ can alternatively be seen to represent a linear map between two finite-dimensional vector spaces, given a basis for each vector space. To see this, we first recall some basic definitions from elementary linear algebra. Let $U$ be an $n$-dimensional vector space over a field $F$ and let $B = \{u_1, \dots, u_n\}$ be an \emph{ordered} basis for $U$, where $u_1 < u_2 < \dots < u_n$. With respect to this basis, we can represent each element $x$ of $U$ as an $n$-tuple $[x]_{B} \defeq (a_1, \dots, a_n) \in F^n$, where $x = a_1 u_1 + \cdots + a_n u_n$ is the unique expression of $x$ in terms of the basis elements of $B$. The scalars $a_i$ are called the \emph{coordinates} of $x$ with respect to the basis $B$ and $[x]_{B}$ is the unique \emph{$B$-coordinate representation of $x$}. It is not hard to see that the map $U \rightarrow F^n$, $x \mapsto [x]_{B}$ is an isomorphism of vector spaces. 

Now consider an $n$-dimensional vector space $U$ and an $m$-dimensional vector space $V$ over the same scalar field $F$. Let $B_U = \{u_1, \dots, u_n\}$ be a basis for $U$ and let $B_V = \{v_1, \dots, v_m\}$ be a basis for $V$. If $T: U \rightarrow V$ is a linear map then we construct an $m \times n$ matrix $A$ as follows. For each $u_i \in B_U$, let $[T(u_i)]_{B_V} = a_{1i} v_1 + \cdots + a_{mi} v_m$ and let $A \defeq (a_{ij})$ denote the matrix obtained by gathering all the coefficients $a_{ij}$. We call $A$ the \emph{matrix representing $T$ with respect to bases $B_U$ and $B_V$}. It can be seen that for any $x \in U$, $[T(x)]_{B_V} = A ([x]_{B_U})$. Observe that here the ordering of each basis is important. That is, changing the ordering of a given basis amounts to permuting the rows and columns of the associated matrix representation.

By this discussion, every linear map can be represented by a matrix, given suitable bases for both its domain and co-domain. Moreover, every matrix can be seen as a representation of some linear map. More specifically, let $A$ be an $m \times n$ matrix over a field $F$. Then $A$ is the matrix of the linear map $T: F^n \rightarrow F^m$, defined for all $x \in F^n$ by $T(x) \defeq A x$, where $x$ is seen as a column vector of length $n$ over $F$. The \emph{image} of $A$ is the image $\{ Ax \sep x \in F^n \} \subseteq F^m$ of the associated linear map and the \emph{null-space} (or \emph{kernel}) of $A$ is $\{ x \in F^n \sep Ax = 0 \} \subseteq F^n$. The \emph{rank} of the matrix $A$ is the dimension of its image and the \emph{nullity} of $A$ is the dimension of its null-space. A fundamental result of elementary linear algebra is the relation
\begin{quote}
	$n$ = dimension of the image of $A$ + dimension of the null-space of $A$,
\end{quote}

\noindent
often referred to as the \emph{rank-nullity theorem}. 


% 
% Unordered matrices
% 
\subsubsection{Matrices and vectors indexed by arbitrary sets}

Rank and nullity are two examples of matrix properties that are in fact properties of the underlying linear map that the matrix represents. The same holds for many common matrix properties that we focus on in linear algebra; for example determinant and singularity. It follows from the above discussion that such natural matrix properties are invariant under permutation of the rows and columns of the matrix, since the associated linear map is invariant under a permutation of the chosen vector space bases. With this in mind, it is natural to consider a more general notion of a matrix, where the rows and columns are indexed by arbitrary \emph{unordered} sets. 

\makebreak

\noindent
Let $R$ be a commutative ring and let $I$, $J$ be finite, non-empty sets. An \emph{$I \times J$ matrix} $A$ over $R$ is a function $A: I \times J \rightarrow R$, where the rows of $A$ are indexed by $I$ and the columns of $A$ are indexed by $J$. We write $A = (a_{ij})$ to denote that $A(i,j) = a_{ij}$ for all $i \in I $ and $j \in J$. If $I = J$ then $A$ is called a \emph{square matrix}. We often identify relations $A \subseteq I \times J$ with the $(0,1)$-matrix defined by the characteristic function of $A$; in this case the actual co-domain is usually clear from the context. If $A$ is an $I \times J$ matrix then the \emph{dimension} of $A$ is $\card{I} \times \card{J}$. 

By taking $I = [m]$ and $J = [n]$ we get the more familiar notion of an ordered $m \times n$ matrix; i.e. a rectangular array of elements consisting of $m$ rows and $n$ columns. Most natural matrix properties, such as determinant and rank over a field, apply directly to matrices indexed by arbitrary unordered sets sets. 

\noindent
We also consider vectors indexed by arbitrary sets. That is, if $I$ is finite and non-empty, then a \emph{vector indexed by $I$} over a commutative ring $R$ is a function $b: I \rightarrow R$. 

\makebreak

\noindent
Addition and multiplication of unordered matrices is defined in exactly the same way as for ordered matrices, except that we now have to ensure that the index sets of the two matrices, and not just their dimension, are matching. That is, if $A$ and $B$ are two $I \times J$ matrices then their sum $A + B$ is the $I \times J$ matrix defined for all $i \in I$ and $j \in J$ by $(A+B)(i,j) \defeq A(i,j) + B(i,j)$. Similarly, if $A$ is an $I \times K$ matrix and $B$ is a $K \times J$ matrix, where all index sets are finite and non-empty, then the product of $A$ and $B$ is the $I \times J$ matrix $AB$ defined for all $i \in I$ and $j \in J$ by $(AB)(i,j) \defeq \sum_{k \in K}A(i,k)B(k,j)$. 


%For a two-sorted $\tau_M$-structure $\mfA = ( (A,R), M , +, \cdot)$ such that $A,R$ are disjoint sets and $(R,+,\cdot)$ is a commutative ring with identity, let  $I^\mfA = \lbrace a \in A : \exists b \in A, r \in R : (a,b,r) \in M \rbrace$ and $J^\mfA = \lbrace b \in A : \exists a \in A, r \in R: (a,b,r) \in M \rbrace$. Then the structure $\mfA$ encodes the $I^\mfA \times J^\mfA$ matrix $M^\mfA$ over $R^\mfA=(R,+,\cdot)$ defined as $M^\mfA(a,b) := \sum_{(a,b,r) \in R} r$ (where the empty sum is considered to be $0 \in R$). A structure $\mfA$ encodes a square matrix if $I^\mfA = J^\mfA$. Let $N$ be a further ternary relation symbol of mixed arity $(2,1)$ and $\tau_{M,N} := \tau_M \cup \lbrace N \rbrace$. Besides the matrix $M^\mfA$, a $\tau_{M,N}$-structure $\mfA$ additionally encodes an $K^\mfA \times L^\mfA$ matrix $N^\mfA$ in totally analogous fashion. Similarly, let $b$ be a binary relation symbol of mixed arity $(1,1)$ and $\tau_{M,b}:= \tau_M \cup \lbrace b \rbrace$, then a $\tau_{M,b}$-structure $\mfA$ additionally encodes a column vector $b^\mfA$. We understand $\tau_{M,b}$-structures $\mfA$ as encoding linear equation systems $\mcS^\mfA$, where $M^\mfA$ is the coefficient matrix and $b^\mfA$ its solution vector.

% --- Systems of equations over groups and rings ------------------------------
\subsubsection{Systems of linear equations over groups and rings}

%\footnote{We can define a system of equations over any finite group $G$, except that when $G$ is non-Abelian then $G$ is not a $\Z$-module. In that case, an equation $a_1 \cdot x_1 + a_2 \cdot x_2 + \cdots + a_m \cdot x_m = g$ has the restriction that $a_i \in \{-1,0,1\}$ for all $i$, where $a_i = 0$ indicates that $x_i$ does not appear in the equation, $a_i = 1$ indicates that $x_i$ does appear in the equation and $a_i = -1$ indicates that the inverse of $x_i$ appears in the equation. For an Abelian group $G$, there is an easy first-order reduction from a system of equations $A \vec x = \vec b$ over $G$ with $\Z$-coefficients to an equivalent system $A' \vec x = \vec b'$ over $G$ where all coefficients are in $\{-1,0,1\}$.}

Let $G$ be a finite Abelian group, written additively with identity $e$. An equation over $G$ is an expression of the form
\begin{equation}
\label{eqn_equation-over-abelian-group}
	\sum_{j \in J} v_j = g
\end{equation}

\noindent 
where $g \in G$, $J$ is finite and non-empty, and each $v_j$ is either a variable $x_j$ or an inverted variable $(-x_j)$. The expression (\ref{eqn_equation-over-abelian-group}) can be \emph{satisfied} if there is an assignment of values from $G$ to the variables so that the equality holds. A system of equations over $G$ is a collection $S$ of equations of this kind. We can assume, without loss of generality, that such a system contains only variables and no inverted variables. Otherwise, we can consider the system of equations obtained from $S$ by replacing every occurence of an inverted variable $(-x_j)$ with a new variable $x_j^{\text{neg}}$ and including an additional equation $x_j + x_j^{\text{neg}} = e$. With this assumption, we can write a system of equations over $G$ as a matrix equation $A \vec x = \vec b$, where $A \in \lbrace 0,1 \rbrace^{I \times J}$, $\vec b \in \struct{G}^I$, $\vec x$ is a $J$-vector of variables taking values in $G$ and $I,J$ are finite non-empty sets. A system $A \vec x = \vec b$ is said to be \emph{solvable} if there is an assignment of values which simultaneously satisfies each equation; that is, if there is a vector $\vec c \in \struct{G}^J$ such that $A \vec c = \vec b$, where matrix multiplication takes place in $G$ as a $\Z$-module. 

More often, we consider equations where the variables are allowed to take values in a commutative ring rather than simply a group. Let $R$ be a commutative ring and write $+$ and $\cdot$ for addition and multiplication in $R$, respectively. A linear equation over $R$ is an expression of the form
\[
	\sum_{j \in J} a_j x_j = b
\]

\noindent 
where $b \in R$ is a constant, each $x_j$ is a variable and each scalar coefficient $a_j$ is an element of $R$. A system of linear equations over $R$ (or \emph{linear system}, for short) is a collection of such expressions; the system is said to be solvable if there is an assignment of the variables to elements in $R$ that simultaneously satisfies each equation. A linear system over a ring can be described succinctly as a matrix equation $A \vec x = \vec b$, where $A \in \struct{R}^{I \times J}$, $\vec b \in \struct{R}^I$, $\vec x$ is a $J$-vector of variables taking values in $R$ and $I,J$ are finite non-empty sets. 
 

==> appendices/les-different-domains-proofs.tex <==
%--------------------------------------------------------------------------
% From ordered non-commutative to cyclic groups
%--------------------------------------------------------------------------

In the following, we give a fixed-point Turing-reduction from solvability over arbitrary ordered finite rings to solvability over cyclic groups of prime-power order.

%\theoremreductionordgenringslcon
\begin{theorem}
$\SolveGeneralOrdRing \fpleqTur \LCON$. 
\end{theorem}

\begin{proof} 
The proof follows the same lines as the proof of
Theorem~\ref{theorem_reduction-ordings-lcon}.
Again, we use the linear order to identify a (minimal) set $\{
g_1, \dots, g_k \} \subseteq R$ which generates the additive
group $(R,+)$ of~$R$ such that $\ord{(g_1)} \divides \ord{(g_2)} \divides
\cdots \divides \ord{(g_k)} := m$ and $(R,+) \cong \langle g_1 \rangle
\oplus
\langle g_2\rangle \oplus \cdots
\oplus \langle g_k\rangle$. We do not require the ring $R$ to contain
a multiplicative identity, so we use the subgroup generated by $g_k$ to
interpret a cyclic group $\Zm{m}$. Accordingly, every element of
$R$ can be represented by a $k$-tuple of elements in $\langle g_k
\rangle =
\Zm{m}$ (where we make use of the fact that $\langle g_i \rangle$ is
isomorphic to a subgroup of $\langle g_k \rangle$ since $\ord{(g_i)}
\divides
\ord{(g_k)}$).

In order to translate the linear system $(A, \fvec b)$ over $R$ into an
equivalent system $(A^\star, \fvec b^\star)$ over $\Zm{m}$ we proceed
as before: firstly, we substitute every variable $x$ ranging over $R$ by
a tuple $(x_1,x_2, \dots, x_k)$ of variables ranging over the appropriate
subgropups of $\Zm{m}$. Secondly, we rewrite all linear terms that occur in
the
equation system with respect to this representation of $(R,+)$. In
contrast to the proof of Theorem~\ref{theorem_reduction-ordings-lcon} we
have to
distinguish between terms $rx=(r_1,\dots,r_k)(x_1,\dots,x_k)$ and
$xr=(x_1,\dots,x_k)(r_1,\dots,r_k)$ for $r \in R$. Observe that, although
formally $\Zm{m}$ is not contained in $R$, it makes sense to speak
of multiplication of elements from $R$ and $\Zm{m}$ ($(R,+)$ is
a $\Zm{m}$-module and we can easily define the corresponding scalar
multiplication in \fp). %as for example for $x, y\in \Zm{m}$ we have 
%\[ x g_i \cdot y g_j =
%\underbrace{(g_i + \cdots + g_i)}\limits_{x\text{-times}}
%\cdot \underbrace{(g_j + \cdots + g_j)}\limits_{y\text{-times}} =
%\underbrace{(g_ig_j + \cdots + g_ig_j)}\limits_{xy\text{-times}} = (xy)
%\cdot (g_ig_j).\]
The remaining steps follow as in the proof
of Theorem~\ref{theorem_reduction-ordings-lcon}.

\end{proof}










==> appendices/linear-algebra-fpc-proofs.tex <==
%--- Size of the general linear group -----------------------------------------
\begin{lemma}
\label{lemma_cardinality-gen-lin-group}
Let $R$ be a finite local ring with maximal ideal $m$ and let $I$  be a finite set of size $n > 0$. If we denote the residue field $R / m$ by $k$ and its cardinality by $q \defeq \card{k}$ then we have
\[ 
	\card{\genl{I}{k}} = q^{n^2} \cdot \prod_{i=0}^{n-1} (1-q^{i-n}) 
	\quad\text{ and }\quad
	\card{\genl{I}{R}} = \card{R}^{n^2} \cdot \prod_{i=0}^{n-1} (1-q^{i-n}).
\]
\end{lemma}

\begin{proof} 
The first equation is common knowledge: An $I \times I$ matrix over $k$ is invertible if and only if its columns are linearly independent. Each set of $i$ linearly independent columns gives rise to $q^i$ different linear combinations. Thus, there remain $(q^{n}  - q^i)$ many linearly independent columns. This counting argument shows that
\begin{align*}
	\card{\genl{I}{k}} &= (q^{n} -1 ) \cdot (q^{n} - q ) \cdot (q^{n} -q^2 ) \cdots (q^{n} -q^{n-1} ) =  \prod_{i=0}^{n-1} (q^{n} - q^i ).
\end{align*}

\noindent
To derive the second equation, consider the canonical group homomorphism $\pi: \genl{I}{R} \ra \genl{I}{k}$. It is easy to see that $\card{\mathrm{ker}(\pi)} = \card{m}^{n^2}$. The fundamental homomorphism theorem thus implies that $\card{\genl{I}{\struct R}} =  {\card{m}^{n^2}} \card{\genl{I}{k}}$ which proves the second identity since $q \cdot \card{m} = \card{R}$.
\end{proof}

%--- Size of the general linear group -----------------------------------------
\lemmaCardinalityGenLin*

\begin{proof} 
By Lemma~\ref{lemma_cardinality-gen-lin-group}, we have an exact expression for the cardinality of $\card{\genl{I}{R}}$ for any non-empty set $I$ and any finite local ring $R$. It is straightforward to verify that the binary encoding of this expression can be formalised by a formula and a number term of fixed-point logic with counting.
\end{proof} 

==> appendices/reductions-to-solvability.tex <==


\setcounter{theorem}{12}


\lemmanormalformles*


\begin{proof}
We describe the interpretation $\mathcal I$ as the composition of
three quantifier-free transformations of linear equation systems. The
first transformation maps a system $(A, \fvec b)$ over $R$ to an
equivalent system $(B, \fvec c)$ over the ring $\Zm m$, where $m$ is
the characteristic of $R$. Secondly, $(B, \fvec c)$ is mapped to an
equivalent system $(C, \fvec 1)$ over $\Zm m$; i.e. to a system where
the right-hand side of each equation is the constant 1. Finally, we
transform $(C, \fvec 1)$ into an equivalent system $(D, \fvec 1)$ over
$\Zm m$, where $D$ is a $\{0,1\}$-matrix.

The first transformation is obtained by the adapting the proof of
Theorem~\ref{theorem_reduction-ordings-lcon}, which gave a fixed-point
reduction from the solvability problem over ordered rings to
solvability over cyclic groups. More specifically, the reduction maps
a linear equation system over an ordered ring $R$ to an equivalent
system over the characteristic subring of $R$, seen as a cyclic group.
Reviewing the proof, it can be seen that first-order quantifiers and
fixed-point operators are only needed for the decomposition of the
ring $R$ into its local summands and, for each local summand, for the
decomposition into a direct sum of cyclic groups. It follows that when
the underlying ring is fixed, as in our case, these decompositions can
be defined by fixed quantifier-free formulae. Hence, there is a
quantifier-free transformation of the system $(A, \fvec b)$ over the
fixed ring $R$ to an equivalent system $(B, \fvec c)$ over the fixed
ring $\Zm m$.

For the second transformation, suppose that $B$ is an $I \times J$
matrix and $\fvec c$ a vector indexed by $I$. We define a new linear
equation system $\struct T$ over $\Zm m$ in which the right-hand side
of every equation is the constant 1. The system $\struct T$ has, in
addition to all the variables that occur in $\struct S$, a new
variable $v_e$ for every $e \in I$ and a new variable $w_r$ for every
$r \in R$. For every element $r \in \Zm m$, we include in $\struct T$
the equation $(1-r)w_1 + w_r= 1$. It can be seen that this subsysem of
equations has a unique solution given by $w_r = r$ for all $r \in \Zm
m$. Finally, for every equation $\sum_{j \in J} B(e,j) \cdot x_j =
\fvec c(e)$ in $\struct S$ (indexed by $e \in I$) we include in
$\struct T$ the two equations $v_e + \sum_{j \in J} B(e,j) \cdot x_j =
1$ and $v_e + w_{\fvec c(e)}= 1$. By solving the latter equation for
$v_e$ and inserting the result into the former equation, it can be
seen that the system $\struct T$ is equivalent to $\struct S$ and can
be written as $C \cdot \fvec x = \fvec 1$, where $C$ is a matrix over
$\Zm m$. 

Finally, we translate the linear equation system $\struct T: C \fvec x
= \fvec 1$ over $\Zm m$ to an equivalent system over $\Zm m$ in which
all scalar coefficients and constant values are either 0 or 1. As a
first step, we translate $\struct T$ to an intermediate system
$\struct U'$, defined as follows. For each variable $v$ in $\struct
T$, the system $\struct U'$ has the $m$ distinct variables $v_0,
\dots, v_{m-1}$ together with equations $v_i = v_j$ for $i\not= j$. We
also include in $\struct U'$ the equation obtained by replacing, in
each equation of $\struct T$, each term of the kind $rv$ by the term
$\sum_{1 \leq i \leq r} v_i$. Since for each $v$, the variables $v_i$
all have to take the same value, it follows that $\struct U'$ is
equivalent to $\struct T$. However, in order to establish our original
claim we need to rewrite the auxiliary equations of the form $v_i =
v_j$ as a set of equations whose right-hand sides are equal to 1. To
achieve this, we introduce a new variable $v_j^-$ for each $v_j$,
together with the equation $v_j + v_j^- + v_1 = 1$. Finally, we
rewrite each equation $v_i = v_j$ as $v_i + v_j^- + v_1 = 1$. It can
be seen that the resulting system $\struct U$ is equivalent to
$\struct U'$ and has the form $D \cdot \fvec x = \fvec 1$, where $D$
is a $\{0,1\}$-matrix. 
\begin{detailedproof}
\medskip

\noindent
Since the ring $R$, and hence also the ring $\Zm m$, is fixed, it can
be seen that all the reductions we have outlined above can be
formalised as quantifier-free reductions, which proves our claim.
\end{detailedproof}
\end{proof}

\setcounter{theorem}{14}

\lemmahermitenormalform*

\begin{proof}
 If $R$ is not a field, fix an element $\pi \in R$ such that the
maximal ideal in $R$ is $m = \pi R$. Then, every element of $R$ can be
represented in the form $\pi^n u$ where $n\geq 0$ and $u \in U(R)$. It
follows that for all elements $r, s \in R$ we have $r \divides s$ or
$s \divides r$. Now, consider the following procedure: In the
remaining $k \times \ell$-matrix, choose an entry $r \in R$ which is
minimal with respect to divisibility and use row and column
permutations to obtain an equivalent $k \times \ell$-matrix $A^\prime$
which has $r$ in the upper left corner, i.e.\ $A^\prime(1,1) = r$.
Then, use the first row to eliminate all other entries in the first
column. After this transformation, the element $r$ still divides every
entry in the resulting matrix, since all of its entries are linear
combinations of entries of $A^\prime$. Proceed with the $(k-1) \times
(\ell -1)$-submatrix which results by deleting the first row and
column
from $A^\prime$.
\end{proof}

\setcounter{theorem}{21}


\begin{lemma}
\label{lemma_appendix-redtosolv-nonppm}
 Let $\mathcal{I}$ be a first-order interpretation of $\vocLinEqRingFixed{\Zm{m}}$ in a signature $\tau$, where $m = p_1^{n_1} \cdots p_k^{n_k}$ for pairwise distinct primes $p_1, \dots, p_k$ and natural numbers $n_1, \dots, n_k \geq 1$. Then there exists a first-order interpretation $\mathcal{J}$ of $\vocLinEqRingFixed{\Zm{m}}$ such that $\qr(\mathcal I) = \qr(\mathcal J)$ and for all $\tau$-structures $\struct{A}$ we have $\mathcal{I}(\struct{A}) \not\in \clsles{R}$ if, and only if, $\mathcal{J}(\struct{A}) \in \clsles{R}$.
\end{lemma}
\begin{proof}
Let $(A, \fvec b)$ be a linear equation system over $\Zm{m}$ with coefficient matrix $A$ and solution vector $\fvec b$. We explain how to transform $(A,\fvec b)$ into a linear equation system $(A^\prime, \fvec b^\prime)$ over $\Zm{m}$, such that $(A, \fvec b)$ is not solvable if, and only if, $(A^\prime, \fvec b^\prime)$ is solvable. From the construction it will become clear that all necessary transformations can be defined from $\mathcal{I}$ without increasing the quantifier-rank of the respective formulas.

First, we use the Chinese remainder theorem and obtain a sequence of linear equations systems $(A_1, \fvec b_1), \dots, (A_k, \fvec b_k)$ over the local rings $\Zm{p_1^{n_1}}, \dots,  \Zm{p_k^{n_k}}$ such that the linear equation system $(A,\fvec b)$ is not solvable if, and only if, for some $1\leq i \leq k$ the linear system $(A_i, \fvec b_i)$ is not solvable. At this point, we apply Lemma \ref{lemma_criterion_non_solvability} to the systems $(A_i, \fvec b_i)$ and obtain new linear equation systems $(A_i^\prime, \fvec b_i^\prime)$ over $\Zm{p_i^{n_i}}$ which are solvable if, and only if, the linear systems $(A_i, \fvec b_i)$ are not solvable. We apply Lemma \ref{lemmanormalformles} to guarantee that all linear systems $(A_i^\prime, \fvec b_i^\prime)$ over $\Zm{p_i^{n_i}}$ are defined with solution vector $\fvec{1}$. 

In order to construct $(A^\prime, \fvec b^\prime)$, it remains to formalize the logical disjunction over  solvability of the linear systems $(A_i^\prime, \fvec b_i^\prime)$ by means of a linear equation system. To this end, we first combine all linear equation systems $(A_i^\prime, \fvec b_i^\prime)$ as independent subsystems in $(A^\prime, \fvec b^\prime)$. For this embedding we use the isomorphisms $(m/p_1^{n_1}\cdots p_{i-1}^{n_{i-1}} p_{i+1}^{n_{i+1}} \cdots p_k^{n_k}) \Zm{m} \simeq \Zm{p_i^{n_i}}$ and (independently) apply Lemma \ref{lemmanormalformles} again to maintain for all  subsystems $(A_i^\prime, \fvec b_i^\prime)$ the solution vector $\fvec{1}$. Now, again independently for each of the linear subsystems  $(A_i^\prime, \fvec b_i^\prime)$, we do the following: We extend each equation by three new variables $x^i$ and $y^i$ and $z^i$ (all with coefficient $1$) and introduce new equations $x^i=(p_1^{n_1-1}\cdots p_k^{n_k-1})$ and  $(p_1^{n_1-1}\cdots p_k^{n_k-1}) y^i = (p_1^{n_1-1}\cdots p_k^{n_k-1})$. These equations guarantee that (in a solution) $y^i = 1 + r(p_1p_2\cdots p_k)$ for some $r \in \Zm{m}$, hence the value of $y^i$ is a unit. Substituting the solution vectors $\fvec{1}$ by the vector containing the entry $p_1^{n_1-1}p_2^{n_2-1} \cdots p_k^{n_k-1}$ only, we thus obtain equivalent linear subsystems~$(A_i^\prime, \fvec b_i^\prime)$. At this point, we remove again all variables $x^i$ from the equations in the subsystem $(A_i^\prime, \fvec b_i^\prime)$ which leaves us with trivially solvable subsystems $(A_i^\prime, \fvec b_i^\prime)$.

Finally, the variables $z^i$ come into play: We extend the system $(A^\prime, \fvec b^\prime)$ by the equation $\sum_i z^i = p_1^{n_1-1} \cdots p_k^{n_k-1}$. This equation guarantees that (in a solution), there is at least one $1 \leq i \leq k$ such that $z^i \not= 0$. We make the following observation: Every element $r \in \Zm{m}$ divides $p_1^{n_1-1} \cdots p_k^{n_k-1}$. For units, this is clear, so let $r \in \Zm{m}$ be a non-unit. Then we can express $r$ as $r=p_1^{l_1} \cdots p_k^{l_k} s$, where $l_1, \dots, l_k \geq 0$, $s$ is co-prime to $m$ and for at least one $1 \leq i \leq k$ we have $l_i \geq 1$. However, since $s$ is a unit in $\Zm{m}$, the claim follows. With this observation it is immediate, that the linear subsystem $(A_i^\prime, \fvec b_i^\prime)$ for which $z^i \not= 0$ has to be solvable. Moreover it is clear, that in the case where $(A_i^\prime, \fvec b_i^\prime)$ is solvable, we can set $z^i = p_1^{n_1-1} \cdots p_k^{n_k-1}$ and $z^j = 0$ for all $j \not=i$ in a solution for $(A_i^\prime, \fvec b_i^\prime)$. 
\end{proof}







==> figures/ring-classes.tex <==
\tikzstyle{vertex}=[
	circle,
	draw=white,
	fill=white,
	minimum size=15pt,
	inner sep=2pt,
	font=\small	
]
\tikzstyle{labels}=[
	circle,
	draw=none,
	fill=none,
	minimum size=5pt,
	inner sep=2pt,
	font=\small
]

\begin{tikzpicture}[
	description/.style={fill=white,inner sep=2pt},
	node distance=1cm,
	transform shape,
	>=stealth',
	shorten >=1pt,
	auto,
	semithick
]


	\node[vertex] (nodeLocal) at (0,0) {};
	\node[labels] (nodeLocalLabel) at (nodeLocal) {local rings};
	
	\node[vertex] (nodeChain) [below of=nodeLocal] {};
	\node[labels] (nodeChainLabel) at (nodeChain) {chain rings};

	\node[vertex] (nodeGalois) [below of=nodeChain] {};
	\node[labels] (nodeGaloisLabel) at (nodeGalois) {Galois rings};

	\node[vertex] (nodeReference) [below of=nodeGalois] {};

	\node[vertex] (nodeField) [left of=nodeReference] {};
	\node[labels] (nodeFieldLabel) at (nodeField) {finite fields};

	\node[vertex] (nodePrimeRing) [right of=nodeReference] {};
	\node[labels] (nodePrimeRingLabel) at (nodePrimeRing) {prime rings};

	% Draw inclusion edges.
	\path[color=black,-] 
		(nodeChain) edge (nodeLocal)
		(nodeGalois) edge (nodeChain)
		(nodeField) edge (nodeGalois)
		(nodePrimeRing) edge (nodeGalois)
		;
\end{tikzpicture}


